A convergent low-wavenumber, high-frequency homogenization of the wave equation in periodic media with a source term

We pursue a low-wavenumber, second-order homogenized solution of the time-harmonic wave equation at both low and high frequency in periodic media with a source term whose frequency resides inside a band gap. Considering the wave motion in an unbounded medium $\mathbb{R}^d$ ($d\geqslant1$), we first use the (Floquet-)Bloch transform to formulate an equivalent variational problem in a bounded domain. By investigating the source term's projection onto certain periodic functions, the second-order model can then be derived via asymptotic expansion of the Bloch eigenfunction and the germane dispersion relationship. We establish the convergence of the second-order homogenized solution, and we include numerical examples to illustrate the convergence result.

==> Arxiv submission R1/mathmacros2.tex <==
%\DeclareMathAlphabet{\itbf}{OML}{cmm}{b}{it}
%\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
%\renewcommand{\hat}{\widehat}
\newcommand{\partD}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\Lk}{{\bf L}(k)}
\newcommand{\tLk}{\tilde{{\bf L}}(k)}
\newcommand{\eps}{\epsilon}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bV}{\boldsymbol{V}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mH}{\boldsymbol{\mathcal{H}}}
%\newcommand{\grad}{\nabla}
\newcommand{\curl}{\nabla \times}
\newcommand{\dive}{\nabla \cdot}
\newcommand{\mdiv}{\mbox{div\,}}
\newcommand{\mcurl}{\mbox{curl\,}}
\newcommand{\mop}{\mbox{op}}
\newcommand{\mOp}{\mbox{Op}}
\newcommand{\ind}{\,\mbox{d}}
\newcommand{\bk}{{\boldsymbol{k}}}
\newcommand{\beps}{{\boldsymbol{\varepsilon}}}
\newcommand{\bgam}{{\boldsymbol{\gamma}}}
\newcommand{\bsig}{{\boldsymbol{\sigma}}}
\newcommand{\bpsi}{{\boldsymbol{\psi}}}
\newcommand{\bmu}{{\boldsymbol{\mu}}}
\newcommand{\brho}{{\boldsymbol{\rho}}}
\newcommand{\bchi}{{\boldsymbol{\chi}}}
\newcommand{\boldeta}{{\boldsymbol{\eta}}}
\newcommand{\balpha}{{\boldsymbol{\alpha}}}
\newcommand{\bzeta}{{\boldsymbol{\zeta}}}
\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bn}{\boldsymbol{n}}
\newcommand{\bj}{\boldsymbol{j}}
\newcommand{\bell}{\boldsymbol{\ell}}
%\newcommand{\bi}{\boldsymbol{i}}

\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bzero}{\boldsymbol{0}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bnu}{\boldsymbol{\nu}}
\newcommand{\vel}{\langle\tilde{\textrm{\slshape{v}}}\rangle}
\newcommand{\tran}{^{\mbox{\tiny T}}}
\newcommand{\hh}{\hspace*{0.7pt}}
\newcommand{\ww}{w}
\newcommand\eqvarm[1]{\stackrel{\var^{#1}}{=}}

\newcommand{\es}{\hspace*{0.7pt}}
\newcommand{\nes}{\hspace*{-0.65pt}}
\newcommand{\wtx}{\tilde{\bx}}
\newcommand{\wtu}{\tilde{u}}

\newcommand{\up}{u^{\mbox{\tiny ($p$)}}}
\newcommand{\Up}{U^{\mbox{\tiny ($p$)}}}


